Automated Evaluation of One-Loop Six-Point Processes for the LHC

In the very near future the first data from LHC will be available. The searches for the Higgs boson and for new physics will require precise predictions both for the signal and the background processes. Tree level calculations typically suffer from large renormalization scale uncertainties. I present an efficient implementation of an algorithm for the automated, Feynman diagram based calculation of one-loop corrections to processes with many external particles. This algorithm has been successfully applied to compute the virtual corrections of the process $u\bar{u}\to b\bar{b}b\bar{b}$ in massless QCD and can easily be adapted for other processes which are required for the LHC.

==> drell-yan/bornsquare.tex <==
\begin{fmfchar*}(60,40)
\fmfleft{q,qb}\fmfright{qc,qbc}\fmftop{tc}\fmfbottom{bc}
\fmfblob{.15w}{blob}
\fmfv{label=$L^{\mu\nu}$,label.angle=60,label.dist=.1w}{blob}
\fmfv{label=$\bar{q}$}{qb}
\fmfv{label=$\bar{q}^\ast$}{qbc}
\fmfv{label=$q^\prime$}{q}
\fmfv{label=$q^{\prime\ast}$}{qc}
\fmfdot{vl,vr}
\fmf{fermion}{q,vl,qb}
\fmf{fermion}{qbc,vr,qc}
\fmf{photon}{vl,blob}
\fmf{photon}{blob,vr}
\fmf{dashes}{tc,bc}
\end{fmfchar*}


==> drell-yan/virtsquare.tex <==
\begin{fmfchar*}(60,40)
\fmfleft{q,qb}\fmfright{qc,qbc}\fmftop{tc}\fmfbottom{bc}
\fmfblob{.15w}{blob}
\fmfv{label=$L^{\mu\nu}$,label.dist=.1w,label.angle=50}{blob}
\fmfv{label=$\bar{q}$}{qb}
\fmfv{label=$\bar{q}^\ast$}{qbc}
\fmfv{label=$q^\prime$}{q}
\fmfv{label=$q^{\prime\ast}$}{qc}
\fmfdot{vl,vr,rho1,rho2}
\fmf{fermion}{q,rho1,vl,rho2,qb}
\fmf{fermion,tension=0.5}{qbc,vr,qc}
\fmf{photon}{vl,blob}
\fmf{photon}{blob,vr}
\fmffreeze
\fmf{gluon,left=.5}{rho1,rho2}
\fmf{dashes}{tc,bc}
\end{fmfchar*}


==> lll.tex <==
For finding the shortest loop the LLL algorithm~\cite{LLL,Mignotte92}
is applied
to the vectors returned by \textsc{Find Loops}.  This step, however, is just
a strategy and not required for the termination of the algorithm; any
selection of a pair of edges \(X\) and \(Y\) that reduces the length of a cycle
is sufficient.
\clearpage

\subsection{The LLL Algorithm}
\TODO{Prove that LLL does not violate $v_i\in{0,\pm1}$, prove that the loop sizes are reduced.}
In 1982 \person{Lenstra}, \person{Lenstra} and \person{Lov\'asz}~\cite{LLL}
proposed and algorithm
which can be used to factorise polynomials with rational coefficients
which is based on the reduction of lattices. For most of the discussion
I follow the notation of~\cite{Hare:1998} where the actual form of
the dot product $\langle\cdot,\cdot\rangle$ and the induced
norm~$\vert\cdot\vert$ remain unspecified, which
allows a wider range of applications than in the original publication.
\begin{definition}[Lattice]\index{Lattice}
A subset $L$ of the $n$-dimensional vector space $\Rset^n$ is called
a lattice if there exists a basis $\{b_1, b_2, \ldots, b_n\}$ of $\Rset^n$
such that
\begin{equation}
L=\sum_{i=1}^n\Zset b_i=\left\{\sum_{i=1}^n z_ib_i: z_i\in\Zset\right\}
\end{equation}
%The determinant of a lattice is defined as
%\begin{equation}
%d(L)\equiv\vert\det(b_1,b_2,\ldots,b_n)\vert
%\end{equation}
%and is independent of the choice of the basis.
\end{definition}

For the discussion of the reduction of loops as described in the
previous section, where each loop is represented as a $\Zset_3$ chain
of vectors $e_i$ denoting the (directed) edges in a graph, requires
the restriction of Lattices to subsets describing $\Zset_3$ chains.
Let us choose $\{-1, 0, 1\}$ as a representant system of $\Zset_3$
then I will call such a subset a \emph{cube} in the rest of the section.
\begin{definition}[Cube]\index{Cube|see{Lattice}}
A subset $C\subset L$ of a lattice is called a cube if its elements $c$
can be written as
\begin{equation}
c=\sum_{i=1}^n c_ib_i\quad\text{with $c_i\in\{-1,0,+1\}$}
\end{equation}
and $b_i$ forming a basis of $L$.
\end{definition}

The problem that the LLL algorithm tries to solve is the reduction
of a lattice basis: if $b_1=(1, 0, 1)$ and $b_2=(20, 1, 19)$ are
two of the basis vectors of a lattice, clearly $b_2$ can be replaced
by $b_2^\prime=b_2-20b_1=(0, 1, -1)$. Intuitively one would find
the second basis simpler than the first one. The notion of
\emph{reducibility} of a lattice basis formalises what is meant
by \emph{simpler} in the above example.
\begin{definition}[Reduced Lattice Basis]\index{Lattice!reduced}
A basis $\{b_1, b_2, \ldots, b_n\}$ of a lattice $L$ is called
reduced if
\begin{equation}
\prod_{i=1}^n\vert b_i\vert\quad\text{is minimal.}
\end{equation}
\end{definition}

The \person{Gram}-\person{Schmidt}
orthogonalisation, where
\begin{subequations}\label{eq:qcd-irreps:gram-schmidt}
\begin{align}
b_i^\ast&=b_i-\sum_{j=1}^{i-1}\mu_{ij}b_j^\ast\quad\text{and}\\
\mu_{ij}&=\frac{\langle b_i,b_j^\ast\rangle}%
{\langle b_j^\ast, b_j^\ast\rangle}\text{,}
\end{align}
\end{subequations}
leads to an orthogonal basis $\{b_1^\ast,\ldots b_n^\ast\}$
and defines the entries of the matrix $\mu_{ij}$ recursively.
It can be shown that applying orthogonalisation to a basis of a
lattice reduces the product
\begin{equation}
\prod_{i=1}^n\vert b_i\vert=
\prod_{i=1}^n\left\vert b_i^\ast+\sum_{j=0}^{i-1}\mu_{ij}b_j^\ast\right\vert
\geq\prod_{i=1}^n\vert b_i^\ast\vert
\end{equation}
since the $b_i^\ast$ form a orthogonal basis. The orthogonal basis,
however, cannot be assumed any longer to form a basis of the lattice.

The authors of~\cite{LLL} introduce a weaker definition of
reducibility of a lattice basis which still retains many of the
properties but can be computed with polynomial complexity.
\begin{definition}[LLL Reduced]\index{LLL reduced}
\label{def:qcd-irrep:LLLreduced}
Let $b_1^\ast,\ldots, b_n^\ast$ be the orthogonalised vectors of
a lattice basis $b_1, \ldots, b_n$ and $\mu_{ij}$ the corresponding
matrix as defined in Equations~\eqref{eq:qcd-irreps:gram-schmidt}.
The basis is called LLL reduced if
\begin{align}
\vert\mu_{ij}\vert\leq\frac12,&\quad\text{for}\quad 1 \leq j < i \leq n
\quad\text{and}\\
\left\vert b_i^\ast\right\vert^2\geq
\left(\frac34-\mu_{i,i-1}^2\right)\left\vert b_{i-1}^\ast\right\vert^2,&%
\quad\text{for}\quad 1 < i \leq n\text{.}
\end{align}
\end{definition}

Algorithm~\ref{alg:qcd-irrep:LLL} reduces a lattice basis in
terms of the Definition~\ref{def:qcd-irrep:LLLreduced}; the proofs
can be found in~\cite{LLL}.
\begin{algorithm}
\caption{LLL Algorithm}\label{alg:qcd-irrep:LLL}
\begin{algorithmic}
\REQUIRE $b_1, b_2, \ldots, b_n$ a lattice basis
\STATE Calculate $b_1^\ast, b_2^\ast, \ldots, b_n^\ast$ and $\mu_{ij}$
from Equations~\eqref{eq:qcd-irreps:gram-schmidt}.
\STATE $B_i\leftarrow \langle b_i^\ast, b_i^\ast\rangle, i=1,\ldots,n$
\STATE $k\leftarrow2$
\WHILE{$k\leq n$}
	\IF{$B_k<(3/4-\mu_{k,k-1}^2)B_{k-1}$}
		\STATE Swap $b_k\leftrightarrow b_{k-1}$
		\STATE Update $b_1^\ast, b_2^\ast, \ldots, b_n^\ast$
		and $\mu_{ij}$.
		\IF{$k>2$} \STATE $k\leftarrow k-1$\ENDIF
	\ELSE
		\FOR{$l\leftarrow k-2$ to $1$ (descending)}
			\IF{$\vert\mu_{kl}\vert>1/2$}
				\STATE $b_k\leftarrow b_k-[\mu_{kl}]b_l$
				\COMMENT{where $[\mu_{kl}]$ denotes the 
					 integer closest to $\mu_{kl}$.}
				\STATE Update
				$b_1^\ast, b_2^\ast, \ldots, b_n^\ast$
				and $\mu_{ij}$.
			\ENDIF
		\ENDFOR
		\STATE $k\leftarrow k+1$
	\ENDIF
\ENDWHILE
\RETURN $b_1, b_2, \ldots, b_n$
\end{algorithmic}
\end{algorithm}

One of the properties of a LLL-reduced basis of a lattice $L$
is that its first vector $b_1$ is minimal in the
following sense~\cite{LLL}:
\begin{equation}\label{eq:qcd-irrep:LLLproperty5}
\vert b_1\vert^2\leq 2^{n-1}\vert x\vert^2,\quad\forall x\in L,
\vert x\vert^2\neq 0\text{.}
\end{equation}
Consider now a $b_1, b_2, \ldots, b_n$ being a LLL reduced
basis of the cycles of a diagram with edges $e_j$, then
the basis vectors are formal sums
\begin{equation}
b_i=\sum_{j=1}^n c_{ij}e_j,\quad c_{ij}\in\{-1, 0, +1\}
\end{equation}
and an inner product can be defined such
that $\langle e_i, e_j\rangle=\delta_{ij}$.
Then $\vert b_i\vert^2$ corresponds to the number of
edges with non-zero entries, hence the length of the
corresponding cycle; the modulus of the
product of two basis vectors $\vert\langle b_i,b_j\rangle\vert$
is the number of edges which the two cycles have in common.
Let $g$ be the girth of the considered
graph, i.e. the length of the shortest cycle.
Equation~\eqref{eq:qcd-irrep:LLLproperty5} then 
implies
\begin{equation}
g\leq b_1\leq 2^{n-1}g
\end{equation}
because the vector $x$ can be chosen to be the shortest
cycle of the graph. If $n=1$ one trivially finds the shortest loop.
For larger graph one only obtains an upper bound on the length of $b_1$
and it remains to be studied if the application of the LLL algorithm
to a cycle basis of a graph always yields the shortest cycle in
$b_1$ and if the returned basis always corresponds to a cube
as defined above. For our application it would be sufficient to
find a proof for cubic graphs for which proofs are easier
than in the general case. 

For the algorithm in Section~\ref{ssec:qcd-irreps:reduce} the selection
of the shortest cycle is not essential and the algorithm terminates even
if a random cycle is reduced in every step. On the other hand the order
in which the reduction is done can well influence the performance of
the algorithm which has not been studied in detail.


==> progress06.tex <==
\chapter*{Outline, Current Progress and Future Plans}
\section{Realm of my Research}
For the year~2008 the start of the~\ac{lhc} is expected providing the community of particle physics with
exciting results; furthermore a strong expectation towards the discovery of new physics already sheds its light
beyond the physics community on the broader publicity. A lot of effort has been spent in understanding new
theories that might extend the standard model. For a successful discovery also the standard model itself has
to be understood on a level of very high precision. Since the \ac{lhc} is a proton collider the main contribution
is expected from~\ac{qcd}.

As an outcome of the Les Houches workshop~2006, the authors of~\cite{Buttar:2006zd} give a list of the most important processes for 
the~\ac{lhc} which are still only known to leading order in~$\alpha_s$; this list includes among others the processes~$pp\rightarrow4\,\text{jets}$,
$pp\rightarrow t\bar{t}b\bar{b}$ and~$pp\rightarrow t\bar{t}+2\,\text{jets}$. These processes have in common
that they require the knowledge of the six-quark
amplitude~$\mathcal{A}(q\bar{q}\rightarrow q^\prime\bar{q}^\prime q^{\prime\prime}\bar{q}^{\prime\prime})$
at~\ac{nlo} in~$\alpha_s$; the calculation of this amplitude is the main topics of my thesis. So far no six-point amplitudes in~\ac{qcd} are
known to~\ac{nlo} precision and hence the calculation of the six-quark amplitude enters a new level of complexity.
The tools and techniques necessary for multi-particle amplitudes at~\ac{nlo} are developed in
collaboration with the~\texttt{GOLEM} working group\footnote{T.~Binoth, A.~Guffanti, J.-Ph.~Guillet, G.~Heinrich, S.~Karg,
N.~Kauer, F.~Mahmoudi, E.~Pilon, T.R., C.~Schubert}
whose aim is the implementation of a general tool for the evaluation of one-loop matrix elements. In parallel to this semi-numerical
approach an algebraical standalone calculation will provide a comparison in terms of efficiency and stability.

The main topics of the applied approach are specified in the following chapter. The amplitude is represented in the
\acl{shp} method and a reduction formalism is applied to the loop integrals such that the helicity amplitudes are given in terms of
a minimal set of basis integrals which in the end are evaluated numerically. The real emission part of the amplitude
is treated by the dipole subtraction method introduced by \person{Catani} et al.~\cite{Catani:2002hc}.

Another more formal topic of my research is the investigation of amplitude properties in the \person{Wess}-\person{Zumino} model. 
Here my work is founded on previous results from my Diploma thesis, where I already calculated the six-scalar amplitude and derived
supersymmetric \person{Ward} identities for amplitudes. These identities relate the bosonic and fermionic fields of the theory and hence
also provide relations between different amplitudes.

\section{Current Status}
During the first phase of my thesis I studied the mathematical background and existing literature
about \ac{qcd}, the method of \acl{shp} and a reduction formalism for one-loop integrals
\cite{Ellis:QCD,Kugo:Gauge,Xu:1987,Dixon:1996wi,Smith:2004ck,Kosower:1990ax,Binoth:1999sp,Binoth:2005ff}.
A mainly automated framework for generating amplitudes in~\ac{qcd} has been established
using \texttt{QGraf} \cite{Nogueira:1991ex} and \texttt{FORM} \cite{Vermaseren:2000nd,Vermaseren:2002}.
\texttt{FORTRAN90} code has been produced for the virtual contribution of the six-quark amplitude, which
uses the~\texttt{GOLEM90} library\footnote{This library is provided by J.-Ph.~Guillet.}
for the numerical evaluation of the basis integrals.
The pieces relevant for the six-quark amplitude are implemented now,
while being debugged and revised in the moment.

\section{Future Plans}
The next step towards a full calculation of the six-quark amplitude is the implementation of the real emission part. The
fully algebraic reduction of the tensor integrals, which will supplement the semi-numeric evaluation, has to be finished.
The code has to be optimised and parallelised because a major
performance increment (with respect to speed and size) is required for the calculation of the full amplitude.
A stable and complete version of the code is expected to be ready in less than one year. This schedule would allow to
present first results at the Les~Houches workshop~2007.

After that step the necessary
adaptions will be made to run the calculation of the six-quark amplitude involving a pair of massive quarks. I expect that
only minor alterations to the code are necessary to allow the calculation of further amplitudes but unforeseen technical
difficulties are very likely in large scale computations and should not be ignored in the schedule.

A publication of the results about the \person{Wess}-\person{Zumino} model is in preparation. 
Further investigations of the supersymmetric \person{Ward} identities
will be made in connection with the \acl{shp} method and depending on these results an application 
for~\ac{qcd} may be considered.






